Are Trees Really Green? A Detection Approach of IoT Malware Attacks

Nowadays, the Internet of Things (IoT) is widely employed, and its usage is growing exponentially because it facilitates remote monitoring, predictive maintenance, and data-driven decision making, especially in the healthcare and industrial sectors. However, IoT devices remain vulnerable due to their resource constraints and difficulty in applying security patches. Consequently, various cybersecurity attacks are reported daily, such as Denial of Service, particularly in IoT-driven solutions. Most attack detection methodologies are based on Machine Learning (ML) techniques, which can detect attack patterns. However, the focus is more on identification rather than considering the impact of ML algorithms on computational resources. This paper proposes a green methodology to identify IoT malware networking attacks based on flow privacy-preserving statistical features. In particular, the hyperparameters of three tree-based models -- Decision Trees, Random Forest and Extra-Trees -- are optimized based on energy consumption and test-time performance in terms of Matthew's Correlation Coefficient. Our results show that models maintain high performance and detection accuracy while consistently reducing power usage in terms of watt-hours (Wh). This suggests that on-premise ML-based Intrusion Detection Systems are suitable for IoT and other resource-constrained devices.

==> figures/pareto_extra_trees.tex <==
\begin{figure}[ht]
    \centering
    \pgfplotsset{colormap={GreenToRed}{rgb255(0cm)=(50, 255, 50); rgb255(1cm)=(255, 69, 0)}}
    \begin{tikzpicture}
        \begin{axis}[axis lines=left, enlargelimits=0.05, grid=both, minor tick num=4, grid style={DimGray, very thin, densely dotted}, major grid style={Black, thick}, minor grid style={}, every axis plot/.append style={thick}, width=0.95\linewidth, height=0.6\linewidth, legend style={at={(0.975, 0.025)}, draw=Gray, anchor=south east}, xlabel={consumption [$\mu$Wh]}, ylabel=MCC]
        \addplot[scatter, only marks, mark=*, mark size=1.25pt, colormap name=GreenToRed, point meta=x] table {
            52.81507180763202 0.5883335378785433
            351.2349020890341 0.5793740570571309
            458.15483152503987 0.5844540585917201
            686.4162179458942 0.5601923378127167
            139.31561459753232 0.5862215985857664
            524.307416639664 0.5798773147788291
            172.1490994283032 0.5880500461848873
            542.3442841114359 0.5783992151990728
            78.2400947439772 0.5775424768348789
            536.4918981322127 0.5811761933733132
            371.88213536166927 0.5823133062840422
            346.75701843491225 0.5878687275600568
            444.04690928660943 0.5810439508112797
            505.9339242045135 0.5564333211320251
            471.79833251227006 0.5812258759027201
            359.8133386088872 0.5772027100982041
            723.9640350731717 0.5766656239767215
            261.1941469014479 0.5759268384772155
            514.0682138358736 0.5816674517775272
            264.53502803597956 0.586607884543423
            75.0135244718198 0.585410160076714
            558.598202810495 0.5889347718505346
            337.2527450470717 0.5825943443523421
            124.41230294038998 0.5983922561609756
            858.9241765449582 0.5743574713638776
            222.68050366919726 0.5802254430431296
            226.15437436786027 0.5774152512808856
            304.9523989305079 0.5704663265521018
            419.87068188601285 0.5817267986527467
            1015.3249606758753 0.5598895848660922
            347.18532605205024 0.5749748275039799
            368.2141223797118 0.5852257843855129
            323.5017027464762 0.5877258293914541
            189.85638416315606 0.5875860983179203
            39.33740190781044 0.5826271771596849
            173.18698286438834 0.5797069272271136
            209.900802999682 0.5819276399137333
            273.9434845994372 0.5734242208653819
            110.73971405477732 0.5623773294192721
            591.5883901038843 0.5754697982558687
            421.787178168701 0.5874433324513556
            266.34231457704595 0.582915649953769
            439.50552905034283 0.5857842288102426
            217.92399772717823 0.6116768761545905
            501.84481758947504 0.5853131352964013
            614.2889882082414 0.582417515965518
            421.827313056991 0.5839956763315631
            200.90142570694132 0.5994730478061028
            400.9845551541975 0.5766303374421559
            49.68780998901614 0.6012407494641241
            198.00803722746292 0.6012703019677464
            390.0366385221735 0.5821705075968661
            126.47450514813609 0.5852513779863651
            294.727534676171 0.5714713710164676
            200.48049770272684 0.5962162111726899
            141.3276587560029 0.5841457439038482
            74.41653905118619 0.5856988313276944
            35.222955561246046 0.5770489775933055
            516.2346724852588 0.5806085536757289
            404.52757254103824 0.5764314932960007
            55.59302360244503 0.5948172556352994
            342.26765309023176 0.5771574497228334
            434.7632088130147 0.6097827820082415
            166.75429812700418 0.5806073345904412
            284.455 0.526
            22.043 0.574
            213.380 0.611
            49.68780998901614 0.6012407494641241
        };
        \addplot[only marks, mark=o, mark size=3pt, thick, draw=Gray] table {
            39.33740190781044 0.5826271771596849
            217.92399772717823 0.6116768761545905
            49.68780998901614 0.6012407494641241
            198.00803722746292 0.6012703019677464
            35.222955561246046 0.5770489775933055
        };
        \addplot[only marks, mark=asterisk, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=DimGray] table {
            284.455 0.526
        };
        \addplot[only marks, mark=+, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=ForestGreen] table {
            22.043 0.574
        };
        \addplot[only marks, mark=x, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=Crimson] table {
            213.380 0.611
        };
        \addplot[only marks, mark=pentagon, mark size=4.5pt, thick, draw=RoyalBlue] table {
            49.68780998901614 0.6012407494641241
        };
        \legend{, Pareto front, default, max green, max MCC, balanced}
        \end{axis}
    \end{tikzpicture}
    \caption{Pareto front for the extra trees.}
    \label{fig:ParetoExtraTrees}
\end{figure}


==> figures/pareto_random_forests.tex <==
\begin{figure}[ht]
    \centering
    \pgfplotsset{colormap={GreenToRed}{rgb255(0cm)=(50, 255, 50); rgb255(1cm)=(255, 69, 0)}}
    \begin{tikzpicture}
        \begin{axis}[axis lines=left, enlargelimits=0.05, grid=both, minor tick num=4, grid style={DimGray, very thin, densely dotted}, major grid style={Black, thick}, minor grid style={}, every axis plot/.append style={thick}, width=0.95\linewidth, height=0.6\linewidth, legend style={at={(0.975, 0.025)}, draw=Gray, anchor=south east}, xlabel={consumption [$\mu$Wh]}, ylabel=MCC]
        \addplot[scatter, only marks, mark=*, mark size=1.25pt, colormap name=GreenToRed, point meta=x] table {
            404.0092940551965 0.5881941933080643
            224.80507333471178 0.5676231655469988
            28.70561167011063 0.6145112008461668
            165.26019068116935 0.5770818398306355
            735.8813852241901 0.5714169595616593
            354.79924262623405 0.5806264220307807
            203.66117337745075 0.57759193765225
            254.65327727898833 0.5806140698559196
            416.8411875355752 0.5926609461209511
            758.6886066783782 0.5711577123950127
            563.962345522764 0.5761513505670112
            95.36690400337443 0.5981320471753484
            199.53702198402848 0.6124116821796212
            156.89207257849608 0.5906928127381409
            904.255761592708 0.5684431849935501
            137.60938185985623 0.5800636189841784
            395.7333002447614 0.583052413234516
            453.21747189301624 0.5800841060726438
            494.4656400699405 0.5811966844817832
            479.61956428197635 0.5784305891035212
            178.12788693361873 0.5972702861651493
            97.09941190578411 0.5747040246787104
            604.6632114886254 0.5757635204138528
            73.62349320529611 0.6102497123955792
            323.58827843734923 0.5759516956971541
            221.94086859087162 0.5771629147659818
            296.7762000126828 0.5769897611481778
            200.32042491077812 0.614824676534387
            184.1972493295689 0.5865372804140802
            379.05131856864006 0.5684769654902544
            280.51769309311516 0.5739442799835248
            384.68736627174474 0.6088398672582876
            768.7778914209181 0.5718945884798604
            672.8657034783917 0.5690811483660763
            195.87895961384555 0.5854785269366437
            344.5337273564585 0.5786297054201931
            122.19510945041365 0.5612095204932042
            396.56070487675606 0.5727897542158719
            516.6080780540686 0.5805998787542166
            483.02931827842707 0.5799696289155066
            208.05634021622242 0.5860434136641712
            347.7865174512493 0.5673435827571999
            542.4675430028981 0.5783921596695396
            404.2128472985247 0.5775075459529744
            186.66408152111094 0.5805349086797255
            270.79536558531123 0.5754450559206092
            261.48766214737697 0.6158171048984926
            372.8581903878158 0.5710155913067269
            280.2855804332998 0.5732470729144518
            378.72424912635194 0.6151157514454232
            291.0118365036173 0.5807213767667582
            161.1744667894042 0.5900618515297816
            216.1759649700172 0.5790059116744983
            664.6306627695396 0.5695225641486727
            309.3320843279826 0.5710102043641437
            329.63294834107444 0.5744949725678383
            191.89205741166856 0.5722455265240642
            154.36569068684582 0.5822129630839455
            29.268010641669978 0.6060993328640922
            463.7847675991582 0.5899311089107198
            277.17502584554364 0.5744387477477118
            115.98474514767699 0.6093081376573503
            175.10713719221826 0.5753662208596594
            105.55045974302917 0.5708706450693717
            299.836 0.524
            22.729 0.582
            124.908 0.616
            28.70561167011063 0.6145112008461668
        };
        \addplot[only marks, mark=o, mark size=3pt, thick, draw=Gray] table {
            28.70561167011063 0.6145112008461668
            200.32042491077812 0.614824676534387
            261.48766214737697 0.6158171048984926
        };
        \addplot[only marks, mark=asterisk, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=DimGray] table {
            299.836 0.524
        };
        \addplot[only marks, mark=+, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=ForestGreen] table {
            22.729 0.582
        };
        \addplot[only marks, mark=x, every mark/.append style={very thick}, mark size=4.5pt, thick, draw=Crimson] table {
            124.908 0.616
        };
        \addplot[only marks, mark=pentagon, mark size=4.5pt, thick, draw=RoyalBlue] table {
            28.70561167011063 0.6145112008461668
        };
        \end{axis}
    \end{tikzpicture}
    \caption{Pareto front for the random forests.}
    \label{fig:Pareto}
\end{figure}


==> sections/appunti_limits-conclusion-fw.tex <==
LIMITS:
- analizzare più scenari (dataset diversi)
- consumo energetico su macchina dove fai deployment (test altra parte risultati fasulli)
- consumo energetico dipende da macchina hardware => metodologia del nostro approccio: nella realtà disaccoppiare addestramento su server e test con consumo energetico in pipeline per epoche training su dispositivo IoT. Col nostro approccio non risparmi su training ma su test, non riduci impatto energetico training ma sul test in modo da poterlo utilizzare su dispositivi IoT. Utilizzare nostro approccio con lavori calcolo consumo su training (OCCHIO DL) in modo da fare retraining periodico del modello per contrastare il temporal drift

Limits and Future Works?

Valutare lifecycle dei modelli, anche in relazione al fatto che i modelli devono essere retrainati per affrontare il drift.


FW:
- testare dispositivi IoT e consumo energetico su loro
- le feature utilizzate permettono anche live forensics (replay attacchi in fase di test) ma impatto consumo energetico maggiore (test per provare a dire "se la tengo accesa live per 24h, rispetto modello non otimizzato, quanto ti fa risparmiare in termini di CO2, watt, soldi ma dipendono da luogo e tempo)
- calcolo consumo energetico di NFStream, di tutto il processo. Ora calcolo energia solo su test, NON su training (forse non consuma più di tanto perchè sono alberi e impieghi meno tempo ad addestrare, con CNN avrebbe più senso perchè ore addestrare)

==> sections/background.tex <==
\section{Background}\label{sec:background}
\todoAll{cosa ha senso mettere nel background? Diego propone di toglierlo. Silvia pensa di spiegare in mezzo paragrafo alcuni concetti base sul command and control, cosa è, come funziona, a cosa serve; e spiegare brevemente la struttura di un traffico rete, brevemente il protocollo utilizzato, soprattutto spiegare la differenza tra flusso e pacchetto.}

==> sections/intro_appunti.tex <==
\section{Introduction}\label{sec:intro}


Approccio AI based cybersecurity in particolare security rete. problema caldo ML enormi richieste computazionali quindi anche energetiche ML. Lavoro nostro provare ad applicare tecniche recenti di ML generico al tema della cybersecurity (detection attacchi di rete, concentrandoci su caso uso specifico C\&C (NO! addestrato su tutte le classi di IoT 23 => utilizzare stesso dataset per addestrare più modelli scegliendo tra precisione e consumo energetico, così deployment su singolo device IoT che è più comodo perchè riduci la latenza, molto leggero computazionalmente e basso consumo energetico con TEST su FW. Addestrare server e testare consumo energetico nel dispositivo IoT) - perchè importante: infezione malware macchine, bloccare exfiltration dati sensibili). Il nostro ragionamento, in determinate casistiche c'è necessità applicazione reale ML bilanciare richiesta computazionale, consumo energetico e accuracy. Avere in teoria difese adattive, capire quando rete non è sotto attacco, consumo energetico ridotto a scapito minore accuracy. Questi modelli adattati in attacco live per arrivare massima accuracy. In questo modo minori costi per le aziende (consumi meno corrente), minor impatto carbonio (quindi minor dispendio aziende carbon credit per emissioni 0) ma comunque con accuracy non sempre 100 elevata ma comunque con livelli di attenzione.

CONTRIBUTION:
- monitor consumo energetico modello ML  
- riduzione sensibile dell'impatto energetico senza diminuire troppo detection, si rimane sempre su detection molto alta ma riducendo di almeno un ordine di grandezza consumi -> con hyperparametri default impatto energetico diminuisce 4 volte
- post-mortem forensics (ma concettualmente supporta anche live forensics, sicuri di aver usato solo feature calcolabili real time, ma bisogna dirlo alla fine) ma consumo energetico tendenzialmente ridotto
- tutti i modelli addestrati, se addestri quello che è più green e accurato, rispetto al modello con hyperp scikit, consuma di meno ed è più accurato

Novelty: consumo energetico (molti articoli fanno detection e molti su IoT), far capire tramite statistiche dimostrare che esiste costo dato da modelli ML. Molti lavori di consumo energetico su reti neurali (noi su alberi)



Command and Control (\ie C\&C or C2C) are one of the most common attacks on 

Our main contribution is the use of features from network traffic statistics of a C\&C for a green and low energy impactant Machine Learning model. In this way the methdology can be used for IoT and mobile applications where the available resources are limited. Not only, our methodology can also be applied to big centers and industries by leading a very low energy consumption (\ie the case of an industry with many network intrusion detection systems based on ML models, in this way the carbon footprint and the energy consumption would be very low). %Moreover, we trained the model on malicious traffic related to $2020$ malware families and tested the performances on more recent samples in order to examine the temporal drift. This means how much the methodology is reliable and accurate during the years and how much it can resist to samples changing over the years. 
The methodology has also been trained on post-mortem data, \ie considering saved and past network capture traffic, but we can apply the detection mechanism on live forensics network attack detection systems. We also focused on privacy preservation data, as we did not consider the request's body in our feature set. 
\todoAll{Write the intro}

\begin{itemize}
    \item[-] importance of IDS
    \item[-] Statistics energy consumption~\cite{Ross2022_postoNoteUK}
\end{itemize}


The rest of the paper is organized as follows. Section~\ref{sec:sota} reviews literature on detecting C\&C malware communication and energy consumption of ML/DL systems, Section~\ref{sec:methodology} describes the dataset, features and employed approaches. Eventually, Section~\ref{sec:results} discusses the results of the classification with respect to performance and energy consumption of the models. Eventually, Section~\ref{sec:discussion} and Section~\ref{sec:conclusion} discuss limitations of the approach and future works.


Appunti GG: No solo cronaca classica risultati (molti articoli ML applicati cybersecurity, abbiamo livello accuracy che becca tot ma alcuni flussi no). MA i flussi che non becchi, quanto sono importanti? Caratterizzare bene i falsi negativi perchè nel nostro contesto abbiamo un IDS che fa soltanto notifica dei flussi sospetti, se non lo configuri per bloccarli in automatico (sistemi attuali industria bassi e poco diffusi, mission critical necessita essere umano per bloccare). Far vedere nel momento in cui cambiamo lo slider da max acc max risparmio energetico, quanto impatta a livello di falsi positivi? quei falsi positivi che cosa sono? a che tipo di attacco corrispondono? in funzione del dataset, esempio c2c tendenzialmente no flusso unico ma N flussi usati da malware esempio text exfiltration. Nel momento in cui flussi completi, alcuni non detectati sistema, ma se uno solo viene identificato, comunque bloccare traffico, quindi peso del falso negativo più basso tendenzialmente. Abbiamo IDS che protegge macchina infettata malware che fa canale c2c con macchina attaccante in un posto nel mondo. Il malware quando fa c2c non fa un canale e una singola connessione tcp sempre aperta per motivo semplice, perchè una sola connessione prima o poi identificata. Quindi quando serve apre connessione, manda comando e poi chiude. Il punto ora è che vogliamo max accuracy ma se perdi qualche flusso in mezzo a tutti non fa niente, l'importante è averne almeno uno identificato per notificare l'analista umano che poi manualmente verificherà. Impatto limitato del falso negativo. Il falso positivo non fa niente, meglio un alert in più anche se non c'è niente che un alert in meno se c'è qualcosa. Nessuno sano di mente minimizza sicurezza per impatto energetico. Quindi dobbiamo fare analisi dei falsi negativi per capire come identifica in base a dataset. Discussion esempio (future work detection live). Caratterizzare falso negativo in base a IP sorgente-destinazione. Capire come creato dataset (ideale scenario ad-hoc con dati reali correlati a descrizione attacco, replay attacco N volte per capire come identifica attacco). Quindi ora, data la cattura, considero tutti falsi negativi, prendo per ogni falso negativo coppia IP sorgete-destinazione e per ogni coppia visualizzo temporalmente quando ho falsi negativi, prendiamo case study dell'impatto di falsi negativi. Se impatto accuracy è principalmente su falsi positivi, non importa. Se variazione delle metriche e matrici confusione è bassa tra green e non-green, non importa. Ragionamento discussion: nel momento in cui vai in modalità green, se becchi attacco, lì cambiare con detection per max accuratezza quindi numero falsi negativi che hai in live non è mai quello dei test nostri con green perchè attacco non isolato (a meno di cose assurde dove quello fa 1 connessione c2c al giorno, sì ma difficile realtà), nel momento in cui prima connessione, modalità full power quindi gli altri li detecta, flusso non isolato per attaccante (mai un singolo flusso) e quindi maggiore del green. Caso interesse: proteggere sistemi IoT (configurazione bassa e prima o poi un malware infetta), li devi beccare e difendere il prima possibile.

==> sections/limits-futurework.tex <==
\section{Discussion}\label{sec:discussion}
\todoAll{Personalmente (Silvia) metterei limiti, future work nelle conclusioni. Sì.}


\todoAll{(by Dani) Toglierei la parte di XAI. SHAP e famiglia per esempio abbiamo visto che non funzionanon troppo bene con questi IDS.}
Future work:
\begin{itemize}
    \item training
    \item raspberry e altre architetture
    \item xai di quali feature dare più consumi rispetto ad altri
    \item altri attacchi
    \item reti neurali
\end{itemize}

==> sections/table_hypeparam_2.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lrrr}
        \toprule
        \textsc{\textbf{model}} & \textsc{\textbf{max depth}} & \textsc{\textbf{min leaf}} & \textsc{\textbf{min split}}\\
        \midrule
        default & $\infty$ & 1 & 2\\
        max MCC & 134 & 1 & 2\\
        balanced & 72 & 2 & 3\\
        \bottomrule
    \end{tabular}
    \caption{CAPTION. After error analysis.}\label{tab:hypeparam:tree_after}
\end{table}
